A Quantum Approach for Stochastic Constrained Binary Optimization

Analytical and practical evidence indicates the advantage of quantum computing solutions over classical alternatives. Quantum-based heuristics relying on the variational quantum eigensolver (VQE) and the quantum approximate optimization algorithm (QAOA) have been shown numerically to generate high-quality solutions to hard combinatorial problems, yet incorporating constraints to such problems has been elusive. To this end, this work puts forth a quantum heuristic to cope with stochastic binary quadratically constrained quadratic programs (QCQP). Identifying the strength of quantum circuits to efficiently generate samples from probability distributions that are otherwise hard to sample from, the variational quantum circuit is trained to generate binary-valued vectors to approximately solve the aforesaid stochastic program. The method builds upon dual decomposition and entails solving a sequence of judiciously modified standard VQE tasks. Tests on several synthetic problem instances using a quantum simulator corroborate the near-optimality and feasibility of the method, and its potential to generate feasible solutions for the deterministic QCQP too.

==> ICASSP - constrained VQE/myabrv.tex <==
%%
%% IEEEabrv.bib
%% 
%% BibTeX bibliography string definitions of the ABBREVIATED titles of
%% IEEE journals and magazines
%% 
%% NOTE: This text file uses UNIX line feed conventions. When (human)
%% reading this file on other platforms, you may have to use a text
%% editor that can handle lines terminated by the UNIX line feed
%% character (0x0A).
%% 
%% This file is designed for bibliography styles that require TSP
%% abbreviated titles and is not for use in bibliographies that
%% require full-length titles.
%% 
%% Version 1.10 (2003/04/02power
)
%% 
%% Composed by Michael Shell
%% 
%% See:
%% http://www.ctan.org/tex-archive/macros/latex/contrib/supported/IEEEtran/
%% for latest version and current contact information.
%%
%% Special thanks to Laura Hyslop of IEEE for her help in obtaining the
%% information needed to compile this file. Also, Volker Kuhlmann kindly
%% provided some corrections and additions.
%%
%%**********************************************************************
%% Legal Notice:
%% This code is offered as-is without any warranty either expressed or
%% implied; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE!
%% User assumes all risk.
%% In no event shall IEEE or any contributor to this code be liable for
%% any damages or losses, including, but not limited to, incidental,
%% consequential, or any other damages, resulting from the use or misuse
%% of any information contained here.
%%
%% This code is distributed under the Perl Artistic License 
%% ( http://language.perl.com/misc/Artistic.html ) 
%% and may be freely used, distributed and modified - subject to the
%% constraints therein.
%% Retain all contribution notices, credits and disclaimers.
%% 
%% All comments are the opinions of their respective authors and are not
%% necessarily endorsed by the IEEE.
%%**********************************************************************
%
%
% USAGE:
% 
% \bibliographystyle{mybstfile} 
% \bibliography{IEEEabrv,mybibfile}
%
% where the IEEE titles in the .bib database entries use the strings
% defined here. e.g.,
%
%
%    journal = IEEE_J_AC,
%
%
% to yield "{IEEE} Trans. Automat. Contr."
%
%
% IEEE uses abbreviated journal titles in their bibliographies -
% this file is suitable for work that is to be submitted to the IEEE.
%
%
% For work that requires full-length titles, you should use the full
% titles provided in the companion file, IEEEfull.bib.
%
%
% ** NOTES **
%
% 1. Journals have been grouped according to subject in order to make it
%    easier to locate and extract the definitions for related journals - 
%    as most works use references that are confined to a single topic.
%    Magazines are listed in straight alphabetical order.
%
% 2. String names are closely based on IEEE's own internal acronyms.
% 
% 3. Abbreviations follow IEEE's style.
%
% 4. Older, out-of-print IEEE titles are included (but not including titles
%    dating prior to IEEE's formation from the IRE and AIEE in 1963).
%
% 5. The following NEW/current journal definitions have been disabled because
%    their abbreviations have not yet been finalized/verified:
%    
%    STRING{IEEE_J_MC         = "{IEEE} Trans. Mobile Comput."}
%    STRING{IEEE_J_JEM        = "{IEEE/TMS} J. Electron. Mater."}
%    STRING{IEEE_J_MCTE       = "{IEEE} Trans. Molecular Cellular Tissue Eng."}
%    STRING{IEEE_J_ESSL       = "{IEEE/ECS} Electrochemical Solid-State Lett."}
%    STRING{IEEE_J_CJECE      = "Canadian J. Elect. Comput. Eng."}
%    
% 6. The following OLD journal definitions have been disabled because
%    their abbreviations have not yet been found/verified:
%
%    STRING{IEEE_J_EWS        = "{IEEE} Trans. Eng. Writing Speech"}
%    STRING{IEEE_J_BCTV       = "{IEEE} Trans. Broadcast Television Receivers"}
%
% If you know what the proper abbreviation is for a string in #5 or #6 above,
% email me and I will correct them in the next release.

%%%%%%%%%%%%%%%%%%%%%%
%% IEEE Conferences %%
%%%%%%%%%%%%%%%%%%%%%%

% power
@STRING{IEEE_C_NAPS   	= "Proc. North American Power Symposium"}
@STRING{IEEE_C_ISGT    	= "Proc. {IEEE} Conf. on Innovative Smart Grid Technologies"}
@STRING{IEEE_C_GM      	= "Proc. {IEEE} Power \& Energy Society General Meeting"}
@STRING{IEEE_C_SGC    	= "Proc. {IEEE} Intl. Conf. on Smart Grid Commun."}
@STRING{PSCC     		= "Proc. Power Syst. Comput. Conf."}
@STRING{C_ALLERTON     = "Proc. Allerton Conf. on Comm., Control, and Computing"}


% signal processing
@STRING{IEEE_C_ICASSP    = "Proc. {IEEE} Intl. Conf. on Acoustics, Speech, and Signal Process."}
@STRING{C_Asilomar    = "Proc. {Asilomar} Conf. on Signals, Syst. and Comput."}
@STRING{IEEE_C_GLOBALSIP    = "Proc. {IEEE} Global Conf. on Signal and Inf. Process."}
@STRING{IEEE_C_CAMSAP    = "Proc. {IEEE} Wkshp. on Comp. Adv. in Multi-Sensor Adaptive Proc."}

% communications

% control
@STRING{IEEE_C_CDC    	= "Proc. {IEEE} Conf. on Decision and Control"}
@STRING{C_ACC			= "Proc. American Control Conf."}

@STRING{JMLR			= "{J. of Machine Learning Research}"}

%%%%%%%%%%%%%%%%%%%
%% IEEE Journals %%
%%%%%%%%%%%%%%%%%%%

% aerospace and military
@STRING{IEEE_J_AES        = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE        = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_ANNE       = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AS         = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE       = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL        = "{IEEE} Trans. Mil. Electron."}



% autos, transportation and vehicles (non-aerospace)
@STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transport. Syst."}
@STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}



% circuits, signals, systems, audio and controls
@STRING{IEEE_J_SPL        = "{IEEE} Signal Process. Lett."}
@STRING{IEEE_J_ASSP       = "{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_AC         = "{IEEE} Trans. Autom. Contr."}
@STRING{IEEE_J_CNS         = "{IEEE} Trans. Control Netw. Syst."}
@STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT         = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST        = "{IEEE} Trans. Contr. Syst. Technol."}
@STRING{IEEE_J_SP         = "{IEEE} Trans. Signal Process."}
@STRING{IEEE_J_STSP       = "{IEEE} J. Sel. Topics Signal Process."}
@STRING{IEEE_J_SU         = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP        = "{IEEE} Trans. Speech Audio Process."}
@STRING{IEEE_J_UE         = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC       = "{IEEE} Trans. Ultrason., Ferroelect., Freq. Contr."}



% communications
@STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC       = "{IEEE} J. Select. Areas Commun."}
@STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}



% components, packaging and manufacturing
@STRING{IEEE_J_ADVP       = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT       = "{IEEE} Trans. Comp., Hybrids, Manufact. Technol."}
@STRING{IEEE_J_CPMTA      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {A}"}
@STRING{IEEE_J_CPMTB      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {B}"}
@STRING{IEEE_J_CPMTC      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {C}"}
@STRING{IEEE_J_CAPT       = "{IEEE} Trans. Comp. Packag. Technol."}
@STRING{IEEE_J_CAPTS      = "{IEEE} Trans. Comp. Packag. Technol."}
@STRING{IEEE_J_CPART      = "{IEEE} Trans. Comp. Parts"}
@STRING{IEEE_J_EPM        = "{IEEE} Trans. Electron. Packag. Manufact."}
@STRING{IEEE_J_MFT        = "{IEEE} Trans. Manufact. Technol."}
@STRING{IEEE_J_PHP        = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP        = "{IEEE} Trans. Parts, Mater., Packag."}



% CAD
@STRING{IEEE_J_TCAD       = "{IEEE} J. Technol. Computer Aided Design"}
@STRING{IEEE_J_CAD        = "{IEEE} Trans. Computer-Aided Design"}



% coding, data, information, knowledge
@STRING{IEEE_J_IT         = "{IEEE} Trans. Inf. Theory"}
@STRING{IEEE_J_KDE        = "{IEEE} Trans. Knowl. Data Eng."}



% computers, computation, networking and software
@STRING{IEEE_J_C          = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_ECOMP      = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_EVC        = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ       = "{IEEE} Trans. Fuzzy Syst."}
% disabled till definition finalized
STRING{IEEE_J_MC          = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_NET        = "{IEEE/ACM} Trans. Netw."}
@STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Netw."}
@STRING{IEEE_J_PDS        = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SE         = "{IEEE} Trans. Softw. Eng."}



% computer graphics, imaging, and multimedia
@STRING{IEEE_J_IP         = "{IEEE} Trans. Image Process."}
@STRING{IEEE_J_MM         = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG        = "{IEEE} Trans. Vis. Comput. Graphics"}



% cybernetics, ergonomics, robots, man-machine, and automation
@STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
@STRING{IEEE_J_RA         = "{IEEE} Trans. Robot. Autom."}
@STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SSC        = "{IEEE} Trans. Syst. Sci. Cybern."}



% earth, wind, fire and water
@STRING{IEEE_J_GE         = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS        = "{IEEE} Trans. Geosci. Remote Sens."}
@STRING{IEEE_J_OE         = "{IEEE} J. Ocean. Eng."}



% education, engineering, history, IEEE, professional
% disabled till definition is verified
STRING{IEEE_J_CJECE       = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC       = "Proc. {IEEE}"}  %%% Proceedings of the IEEE 
@STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM         = "{IEEE} Trans. Eng. Manage."}
% disabled till definition is verified
STRING{IEEE_J_EWS         = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}



% electromagnetics, antennas, EMI, magnetics and microwave
@STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propagat. Lett."}
@STRING{IEEE_J_MGWL       = "{IEEE} Microwave Guided Wave Lett."}
% IEEE seems to want "Compon." here, not "Comp."
@STRING{IEEE_J_MWCL       = "{IEEE} Microwave Wireless Compon. Lett."}
@STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas Propagat."}
@STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT        = "{IEEE} Trans. Microwave Theory Tech."}
@STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J. Magn. Jpn."}



% energy and power
@STRING{IEEE_J_EC         = "{IEEE} Trans. Energy Convers."}	% 2.43
@STRING{IEEE_J_PWRAS      = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD       = "{IEEE} Trans. Power Del."}	% 1.52 	
@STRING{IEEE_J_PWRE       = "{IEEE} Trans. Power Electron."}	% 4.08
@STRING{IEEE_J_PWRS       = "{IEEE} Trans. Power Syst."}		% 2.92
@STRING{IEEE_J_SG 	      = "{IEEE} Trans. Smart Grid"}
@STRING{IEEE_J_STE 	      = "{IEEE} Trans. Sustain. Energy"}


% industrial, commercial and consumer
@STRING{IEEE_J_APPIND     = "{IEEE} Trans. Applicat. Ind."}
@STRING{IEEE_J_BC         = "{IEEE} Trans. Broadcast."}
% disabled till definition is verified
STRING{IEEE_J_BCTV        = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE         = "{IEEE} Trans. Consumer Electron."}
@STRING{IEEE_J_IE         = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI       = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Applicat."}
@STRING{IEEE_J_IGA        = "{IEEE} Trans. Ind. Gen. Applicat."}



% instrumentation and measurement
@STRING{IEEE_J_IM         = "{IEEE} Trans. Instrum. Meas."}



% insulation and materials
% disabled till definition finalized
STRING{IEEE_J_JEM         = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI        = "{IEEE} Trans. Dielect. Elect. Insulation"}
@STRING{IEEE_J_EI         = "{IEEE} Trans. Elect. Insulation"}



% mechanical
@STRING{IEEE_J_MECH       = "{IEEE/ASME} Trans. Mechatron."}
@STRING{IEEE_J_MEMS       = "J. Microelectromech. Syst."}



% medical and biological
@STRING{IEEE_J_BME        = "{IEEE} Trans. Biomed. Eng."}
% Note: The B-ME journal later dropped the hyphen and became the BME.
@STRING{IEEE_J_B-ME       = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_BMELC      = "{IEEE} Trans. Bio-Med. Electron."}
@STRING{IEEE_J_ITBM       = "{IEEE} Trans. Inf. Technol. Biomed."}
@STRING{IEEE_J_ME         = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI         = "{IEEE} Trans. Med. Imag."}
% disabled till definition finalized
STRING{IEEE_J_MCTE        = "{IEEE} Trans. Molecular Cellular Tissue Eng."}
@STRING{IEEE_J_NB         = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE       = "{IEEE} Trans. Neural Syst. Rehab. Eng."}
@STRING{IEEE_J_RE         = "{IEEE} Trans. Rehab. Eng."}



% optics, lightwave and photonics
@STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_JLT        = "J. Lightwave Technol."}



% physics, electrons, nanotechnology, nuclear and quantum electronics
@STRING{IEEE_J_EDL        = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_JQE        = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE      = "{IEEE} J. Select. Topics Quantum Electron."}
@STRING{IEEE_J_ED         = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO       = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS         = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS         = "{IEEE} Trans. Plasma Sci."}



% reliability
% IEEE seems to want "Mat." here, not "Mater."
@STRING{IEEE_J_DMR        = "{IEEE} Trans. Device Mat. Rel."}
@STRING{IEEE_J_R          = "{IEEE} Trans. Rel."}



% semiconductors, superconductors, electrochemical and solid state
% disabled till definition finalized
STRING{IEEE_J_ESSL        = "{IEEE/ECS} Electrochemical Solid-State Lett."}
@STRING{IEEE_J_JSSC       = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC        = "{IEEE} Trans. Appl. Superconduct."}
@STRING{IEEE_J_SM         = "{IEEE} Trans. Semiconduct. Manufact."}



% sensors
@STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}



% VLSI
@STRING{IEEE_J_VLSI       = "{IEEE} Trans. {VLSI} Syst."}





%%%%%%%%%%%%%%%%%%%%
%% IEEE Magazines %%
%%%%%%%%%%%%%%%%%%%%


@STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag"}
@STRING{IEEE_M_HIST       = "{IEEE} Annals Hist. Comput."}
@STRING{IEEE_M_AP         = "{IEEE} Antennas Propagat. Mag."}
@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}
% CSEM changed to CSE in 1999
@STRING{IEEE_M_CSE        = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C          = "{IEEE} Computer"}
@STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EXP        = "{IEEE} Expert"}
@STRING{IEEE_M_IA         = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IM         = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
@STRING{IEEE_M_MW         = "{IEEE} Microwave"}
@STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
@STRING{IEEE_M_NET        = "{IEEE} Network"}
% IEEE's editorial manual lists "Pers. Commun.", 
% but "Personal Commun. Mag." seems to be what is used in the journals
@STRING{IEEE_M_PCOM       = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_POT        = "{IEEE} Potentials"}
% CAP and PER merged to form PE in 2003
@STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_RA         = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SP         = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S          = "{IEEE} Softw."}
@STRING{IEEE_M_SPECT      = "{IEEE} Spectr."}
@STRING{IEEE_M_TS         = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_WC         = "{IEEE} Wireless Commun. Mag."}
@STRING{IEEE_M_TODAY      = "Today's Eng."}




%--
%EOF


==> ICASSP - constrained VQE/stylesV2.tex <==
% function definitions
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\nullspace}{null}
\DeclareMathOperator{\pr}{Pr}
\DeclareMathOperator{\Beta}{B}
\DeclareMathOperator{\diag}{dg}
\DeclareMathOperator{\bdiag}{bdg}
\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator{\vectorize}{vec}
\DeclareMathOperator{\real}{Re}
\DeclareMathOperator{\imag}{Im}
\DeclareMathOperator{\maximum}{max}
\DeclareMathOperator{\minimum}{min}
\DeclareMathOperator{\signum}{sign}
\DeclareMathOperator{\MLE}{MLE}
\DeclareMathOperator{\subjectto}{s.to}
\DeclareMathOperator{\prox}{prox}
\DeclareMathOperator{\dimension}{dim}
\DeclareMathOperator*{\find}{find}
%\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
%\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

% theorem environments
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

% colored text
\newcommand\cmr[1]{\textcolor{red}{#1}}
\newcommand\cmb[1]{\textcolor{blue}{#1}}
\newcommand\cmg[1]{\textcolor{green}{#1}}

% % all definitions go in the order
% - numbers
% - small Latin letters
% - capital Latin letters
% - small Greek letters
% - capital Greek letters


%%%% BOLD
\newcommand \bzero{\mathbf{0}}
\newcommand \bone{\mathbf{1}}
\newcommand \ba{\mathbf{a}}
\newcommand \bb{\mathbf{b}}
\newcommand \bc{\mathbf{c}}
\newcommand \bd{\mathbf{d}}
\newcommand \be{\mathbf{e}}
\newcommand \bef{\mathbf{f}} % exception since \bf is taken
\newcommand \bg{\mathbf{g}}
\newcommand \bh{\mathbf{h}}
\newcommand \bi{\mathbf{i}}
\newcommand \bj{\mathbf{j}}
\newcommand \bk{\mathbf{k}}
\newcommand \bdell{\boldsymbol{\ell}} % \bell is already taken
\newcommand \bm{\mathbf{m}}
\newcommand \bn{\mathbf{n}}
\newcommand \bo{\mathbf{o}}
\newcommand \bp{\mathbf{p}}
\newcommand \bq{\mathbf{q}}
\newcommand \br{\mathbf{r}}
\newcommand \bs{\mathbf{s}}
\newcommand \bt{\mathbf{t}}
\newcommand \bu{\mathbf{u}}
\newcommand \bv{\mathbf{v}}
\newcommand \bw{\mathbf{w}}
\newcommand \bx{\mathbf{x}}
\newcommand \by{\mathbf{y}}
\newcommand \bz{\mathbf{z}}
\newcommand \bA{\mathbf{A}}
\newcommand \bB{\mathbf{B}}
\newcommand \bC{\mathbf{C}}
\newcommand \bD{\mathbf{D}}
\newcommand \bE{\mathbf{E}}
\newcommand \bF{\mathbf{F}}
\newcommand \bG{\mathbf{G}}
\newcommand \bH{\mathbf{H}}
\newcommand \bI{\mathbf{I}}
\newcommand \bJ{\mathbf{J}}
\newcommand \bK{\mathbf{K}}
\newcommand \bL{\mathbf{L}}
\newcommand \bM{\mathbf{M}}
\newcommand \bN{\mathbf{N}}
\newcommand \bO{\mathbf{O}}
\newcommand \bP{\mathbf{P}}
\newcommand \bQ{\mathbf{Q}}
\newcommand \bR{\mathbf{R}}
\newcommand \bS{\mathbf{S}}
\newcommand \bT{\mathbf{T}}
\newcommand \bU{\mathbf{U}}
\newcommand \bV{\mathbf{V}}
\newcommand \bW{\mathbf{W}}
\newcommand \bX{\mathbf{X}}
\newcommand \bY{\mathbf{Y}}
\newcommand \bZ{\mathbf{Z}}
\newcommand \balpha{\boldsymbol{\alpha}}
\newcommand \bbeta{\boldsymbol{\beta}}
\newcommand \bgamma{\boldsymbol{\gamma}}
\newcommand \bdelta{\boldsymbol{\delta}}
\newcommand \bepsilon{\boldsymbol{\epsilon}}
\newcommand \bzeta{\boldsymbol{\zeta}}
\newcommand \bdeta{\boldsymbol{\eta}} %% bdeta to differentiate from beta
\newcommand \btheta{\boldsymbol{\theta}}
\newcommand \biota{\boldsymbol{\iota}}
\newcommand \bkappa{\boldsymbol{\kappa}}
\newcommand \blambda{\boldsymbol{\lambda}}
\newcommand \bmu{\boldsymbol{\mu}}
\newcommand \bnu{\boldsymbol{\nu}}
\newcommand \bxi{\boldsymbol{\xi}}
\newcommand \bpi{\boldsymbol{\pi}}
\newcommand \brho{\boldsymbol{\rho}}
\newcommand \bsigma{\boldsymbol{\sigma}}
\newcommand \btau{\boldsymbol{\tau}}
\newcommand \bupsilon{\boldsymbol{\upsilon}}
\newcommand \bphi{\boldsymbol{\phi}}
\newcommand \bchi{\boldsymbol{\chi}}
\newcommand \bpsi{\boldsymbol{\psi}}
\newcommand \bomega{\boldsymbol{\omega}}
\newcommand \bGamma{\mathbf{\Gamma}}
\newcommand \bDelta{\mathbf{\Delta}}
\newcommand \bTheta{\mathbf{\Theta}}
\newcommand \bvarTheta{\boldsymbol{\varTheta}}
\newcommand \bLambda{\mathbf{\Lambda}}
\newcommand \bXi{\mathbf{\Xi}}
\newcommand \bPi{\mathbf{\Pi}}
\newcommand \bSigma{\mathbf{\Sigma}}
\newcommand \bPhi{\mathbf{\Phi}}
\newcommand \bPsi{\mathbf{\Psi}}
\newcommand \bOmega{\mathbf{\Omega}}


%%%% TILDE
\newcommand \tda{\tilde{a}}
\newcommand \tdb{\tilde{b}}
\newcommand \tdc{\tilde{c}}
\newcommand \tdd{\tilde{d}}
\newcommand \tde{\tilde{e}}
\newcommand \tdf{\tilde{f}}
\newcommand \tdh{\tilde{h}}
\newcommand \tdi{\tilde{i}}
\newcommand \tdj{\tilde{j}}
\newcommand \tdk{\tilde{k}}
\newcommand \tdell{\tilde{\ell}}
\newcommand \tdm{\tilde{m}}
\newcommand \tdn{\tilde{n}}
\newcommand \tdo{\tilde{o}}
\newcommand \tdp{\tilde{p}}
\newcommand \tdq{\tilde{q}}
\newcommand \tdr{\tilde{r}}
\newcommand \tds{\tilde{s}}
\newcommand \tdt{\tilde{t}}
\newcommand \tdu{\tilde{u}}
\newcommand \tdv{\tilde{v}}
\newcommand \tdw{\tilde{w}}
\newcommand \tdx{\tilde{x}}
\newcommand \tdy{\tilde{y}}
\newcommand \tdz{\tilde{z}}
\newcommand \tdA{\tilde{A}}
\newcommand \tdB{\tilde{B}}
\newcommand \tdC{\tilde{C}}
\newcommand \tdD{\tilde{D}}
\newcommand \tdE{\tilde{E}}
\newcommand \tdF{\tilde{F}}
\newcommand \tdG{\tilde{G}}
\newcommand \tdH{\tilde{H}}
\newcommand \tdI{\tilde{I}}
\newcommand \tdK{\tilde{K}}
\newcommand \tdL{\tilde{L}}
\newcommand \tdM{\tilde{M}}
\newcommand \tdN{\tilde{N}}
\newcommand \tdO{\tilde{O}}
\newcommand \tdP{\tilde{P}}
\newcommand \tdQ{\tilde{Q}}
\newcommand \tdR{\tilde{R}}
\newcommand \tdS{\tilde{S}}
\newcommand \tdT{\tilde{T}}
\newcommand \tdU{\tilde{U}}
\newcommand \tdV{\tilde{V}}
\newcommand \tdW{\tilde{W}}
\newcommand \tdX{\tilde{X}}
\newcommand \tdY{\tilde{Y}}
\newcommand \tdZ{\tilde{Z}}
\newcommand \tdalpha{\tilde{\alpha}}
\newcommand \tdbeta{\tilde{\beta}}
\newcommand \tdgamma{\tilde{\gamma}}
\newcommand \tddelta{\tilde{\delta}}
\newcommand \tdepsilon{\tilde{\epsilon}}
\newcommand \tdzeta{\tilde{\zeta}}
\newcommand \tdeta{\tilde{\eta}}
\newcommand \tdtheta{\tilde{\theta}}
\newcommand \tdiota{\tilde{\iota}}
\newcommand \tdkappa{\tilde{\kappa}}
\newcommand \tdlambda{\tilde{\lambda}}
\newcommand \tdmu{\tilde{\mu}}
\newcommand \tdnu{\tilde{\nu}}
\newcommand \tdxi{\tilde{\xi}}
\newcommand \tdpi{\tilde{\pi}}
\newcommand \tdrho{\tilde{\rho}}
\newcommand \tdsigma{\tilde{\sigma}}
\newcommand \tdtau{\tilde{\tau}}
\newcommand \tdupsilon{\tilde{\upsilon}}
\newcommand \tdphi{\tilde{\phi}}
\newcommand \tdchi{\tilde{\chi}}
\newcommand \tdpsi{\tilde{\psi}}
\newcommand \tdomega{\tilde{\omega}}
\newcommand \tdGamma{\tilde{\Gamma}}
\newcommand \tdDelta{\tilde{\Delta}}
\newcommand \tdTheta{\tilde{\Theta}}
\newcommand \tdLambda{\tilde{\Lambda}}
\newcommand \tdXi{\tilde{\Xi}}
\newcommand \tdPi{\tilde{\Pi}}
\newcommand \tdSigma{\tilde{\Sigma}}
\newcommand \tdPhi{\tilde{\Phi}}
\newcommand \tdPsi{\tilde{\Psi}}
\newcommand \tdOmega{\tilde{\Omega}}

%%%% HAT
\newcommand \hta{\hat{a}}
\newcommand \htb{\hat{b}}
\newcommand \htc{\hat{c}}
\newcommand \htd{\hat{d}}
\newcommand \hte{\hat{e}}
\newcommand \htf{\hat{f}}
\newcommand \hth{\hat{h}}
\newcommand \hti{\hat{i}}
\newcommand \htj{\hat{j}}
\newcommand \htk{\hat{k}}
\newcommand \htell{\hat{\ell}}
\newcommand \htm{\hat{m}}
\newcommand \htn{\hat{n}}
\newcommand \hto{\hat{o}}
\newcommand \htp{\hat{p}}
\newcommand \htq{\hat{q}}
\newcommand \htr{\hat{r}}
\newcommand \hts{\hat{s}}
\newcommand \htt{\hat{t}}
\newcommand \htu{\hat{u}}
\newcommand \htv{\hat{v}}
\newcommand \htw{\hat{w}}
\newcommand \htx{\hat{x}}
\newcommand \hty{\hat{y}}
\newcommand \htz{\hat{z}}
\newcommand \htA{\hat{A}}
\newcommand \htB{\hat{B}}
\newcommand \htC{\hat{C}}
\newcommand \htD{\hat{D}}
\newcommand \htE{\hat{E}}
\newcommand \htF{\hat{F}}
\newcommand \htG{\hat{G}}
\newcommand \htH{\hat{H}}
\newcommand \htI{\hat{I}}
\newcommand \htK{\hat{K}}
\newcommand \htL{\hat{L}}
\newcommand \htM{\hat{M}}
\newcommand \htN{\hat{N}}
\newcommand \htO{\hat{O}}
\newcommand \htP{\hat{P}}
\newcommand \htQ{\hat{Q}}
\newcommand \htR{\hat{R}}
\newcommand \htS{\hat{S}}
\newcommand \htT{\hat{T}}
\newcommand \htU{\hat{U}}
\newcommand \htV{\hat{V}}
\newcommand \htW{\hat{W}}
\newcommand \htX{\hat{X}}
\newcommand \htY{\hat{Y}}
\newcommand \htZ{\hat{Z}}
\newcommand \htalpha{\hat{\alpha}}
\newcommand \htbeta{\hat{\beta}}
\newcommand \htgamma{\hat{\gamma}}
\newcommand \htdelta{\hat{\delta}}
\newcommand \htepsilon{\hat{\epsilon}}
\newcommand \htzeta{\hat{\zeta}}
\newcommand \htdeta{\hat{\eta}} %% bdeta to differentiate from beta
\newcommand \httheta{\hat{\theta}}
\newcommand \htiota{\hat{\iota}}
\newcommand \htkappa{\hat{\kappa}}
\newcommand \htlambda{\hat{\lambda}}
\newcommand \htmu{\hat{\mu}}
\newcommand \htnu{\hat{\nu}}
\newcommand \htxi{\hat{\xi}}
\newcommand \htpi{\hat{\pi}}
\newcommand \htrho{\hat{\rho}}
\newcommand \htsigma{\hat{\sigma}}
\newcommand \httau{\hat{\tau}}
\newcommand \htupsilon{\hat{\upsilon}}
\newcommand \htphi{\hat{\phi}}
\newcommand \htchi{\hat{\chi}}
\newcommand \htpsi{\hat{\psi}}
\newcommand \htomega{\hat{\omega}}
\newcommand \htGamma{\hat{\Gamma}}
\newcommand \htDelta{\hat{\Delta}}
\newcommand \htTheta{\hat{\Theta}}
\newcommand \htLambda{\hat{\Lambda}}
\newcommand \htXi{\hat{\Xi}}
\newcommand \htPi{\hat{\Pi}}
\newcommand \htSigma{\hat{\Sigma}}
\newcommand \htPhi{\hat{\Phi}}
\newcommand \htPsi{\hat{\Psi}}
\newcommand \htOmega{\hat{\Omega}}

%%%% CHECK
\newcommand \cha{\check{a}}
\newcommand \chb{\check{b}}
\newcommand \chc{\check{c}}
\newcommand \chd{\check{d}}
\newcommand \che{\check{e}}
\newcommand \chf{\check{f}}
\newcommand \chh{\check{h}}
\newcommand \chj{\check{j}}
\newcommand \chk{\check{k}}
\newcommand \chell{\check{\ell}}
\newcommand \chm{\check{m}}
\newcommand \chn{\check{n}}
\newcommand \cho{\check{o}}
\newcommand \chp{\check{p}}
\newcommand \chq{\check{q}}
\newcommand \chr{\check{r}}
\newcommand \chs{\check{s}}
\newcommand \cht{\check{t}}
\newcommand \chu{\check{u}}
\newcommand \chv{\check{v}}
\newcommand \chw{\check{w}}
\newcommand \chx{\check{x}}
\newcommand \chy{\check{y}}
\newcommand \chz{\check{z}}
\newcommand \chA{\check{A}}
\newcommand \chB{\check{B}}
\newcommand \chC{\check{C}}
\newcommand \chD{\check{D}}
\newcommand \chE{\check{E}}
\newcommand \chF{\check{F}}
\newcommand \chG{\check{G}}
\newcommand \chH{\check{H}}
\newcommand \chI{\check{I}}
\newcommand \chK{\check{K}}
\newcommand \chL{\check{L}}
\newcommand \chM{\check{M}}
\newcommand \chN{\check{N}}
\newcommand \chO{\check{O}}
\newcommand \chP{\check{P}}
\newcommand \chQ{\check{Q}}
\newcommand \chR{\check{R}}
\newcommand \chS{\check{S}}
\newcommand \chT{\check{T}}
\newcommand \chU{\check{U}}
\newcommand \chV{\check{V}}
\newcommand \chW{\check{W}}
\newcommand \chX{\check{X}}
\newcommand \chY{\check{Y}}
\newcommand \chZ{\check{Z}}
\newcommand \chalpha{\check{\alpha}}
\newcommand \chbeta{\check{\beta}}
\newcommand \chgamma{\check{\gamma}}
\newcommand \chdelta{\check{\delta}}
\newcommand \chepsilon{\check{\epsilon}}
\newcommand \chzeta{\check{\zeta}}
\newcommand \chdeta{\check{\eta}} %% bdeta to differentiate from beta
\newcommand \chtheta{\check{\theta}}
\newcommand \chiota{\check{\iota}}
\newcommand \chkappa{\check{\kappa}}
\newcommand \chlambda{\check{\lambda}}
\newcommand \chmu{\check{\mu}}
\newcommand \chnu{\check{\nu}}
\newcommand \chxi{\check{\xi}}
\newcommand \chpi{\check{\pi}}
\newcommand \chrho{\check{\rho}}
\newcommand \chsigma{\check{\sigma}}
\newcommand \chtau{\check{\tau}}
\newcommand \chupsilon{\check{\upsilon}}
\newcommand \chphi{\check{\phi}}
\newcommand \chchi{\check{\chi}}
\newcommand \chpsi{\check{\psi}}
\newcommand \chomega{\check{\omega}}
\newcommand \chGamma{\check{\Gamma}}
\newcommand \chDelta{\check{\Delta}}
\newcommand \chTheta{\check{\Theta}}
\newcommand \chLambda{\check{\Lambda}}
\newcommand \chXi{\check{\Xi}}
\newcommand \chPi{\check{\Pi}}
\newcommand \chSigma{\check{\Sigma}}
\newcommand \chPhi{\check{\Phi}}
\newcommand \chPsi{\check{\Psi}}
\newcommand \chOmega{\check{\Omega}}


%%%% MATHCAL
\newcommand \mcA{\mathcal{A}}
\newcommand \mcB{\mathcal{B}}
\newcommand \mcC{\mathcal{C}}
\newcommand \mcD{\mathcal{D}}
\newcommand \mcE{\mathcal{E}}
\newcommand \mcF{\mathcal{F}}
\newcommand \mcG{\mathcal{G}}
\newcommand \mcH{\mathcal{H}}
\newcommand \mcI{\mathcal{I}}
\newcommand \mcK{\mathcal{K}}
\newcommand \mcL{\mathcal{L}}
\newcommand \mcM{\mathcal{M}}
\newcommand \mcN{\mathcal{N}}
\newcommand \mcO{\mathcal{O}}
\newcommand \mcP{\mathcal{P}}
\newcommand \mcQ{\mathcal{Q}}
\newcommand \mcR{\mathcal{R}}
\newcommand \mcS{\mathcal{S}}
\newcommand \mcT{\mathcal{T}}
\newcommand \mcU{\mathcal{U}}
\newcommand \mcV{\mathcal{V}}
\newcommand \mcW{\mathcal{W}}
\newcommand \mcX{\mathcal{X}}
\newcommand \mcY{\mathcal{Y}}
\newcommand \mcZ{\mathcal{Z}}

%%%% BAR-MATHCAL (complements of sets)
\newcommand \bmcA{\bar{\mathcal{A}}}
\newcommand \bmcB{\bar{\mathcal{B}}}
\newcommand \bmcC{\bar{\mathcal{C}}}
\newcommand \bmcD{\bar{\mathcal{D}}}
\newcommand \bmcE{\bar{\mathcal{E}}}
\newcommand \bmcF{\bar{\mathcal{F}}}
\newcommand \bmcG{\bar{\mathcal{G}}}
\newcommand \bmcH{\bar{\mathcal{H}}}
\newcommand \bmcI{\bar{\mathcal{I}}}
\newcommand \bmcJ{\bar{\mathcal{J}}}
\newcommand \bmcK{\bar{\mathcal{K}}}
\newcommand \bmcL{\bar{\mathcal{L}}}
\newcommand \bmcM{\bar{\mathcal{M}}}
\newcommand \bmcN{\bar{\mathcal{N}}}
\newcommand \bmcO{\bar{\mathcal{O}}}
\newcommand \bmcP{\bar{\mathcal{P}}}
\newcommand \bmcQ{\bar{\mathcal{Q}}}
\newcommand \bmcR{\bar{\mathcal{R}}}
\newcommand \bmcS{\bar{\mathcal{S}}}
\newcommand \bmcT{\bar{\mathcal{T}}}
\newcommand \bmcU{\bar{\mathcal{U}}}
\newcommand \bmcV{\bar{\mathcal{V}}}
\newcommand \bmcW{\bar{\mathcal{W}}}
\newcommand \bmcX{\bar{\mathcal{X}}}
\newcommand \bmcY{\bar{\mathcal{Y}}}
\newcommand \bmcZ{\bar{\mathcal{Z}}}

%%%% TILDE-MATHCAL
\newcommand \tmcA{\tilde{\mathcal{A}}}
\newcommand \tmcB{\tilde{\mathcal{B}}}
\newcommand \tmcC{\tilde{\mathcal{C}}}
\newcommand \tmcD{\tilde{\mathcal{D}}}
\newcommand \tmcE{\tilde{\mathcal{E}}}
\newcommand \tmcF{\tilde{\mathcal{F}}}
\newcommand \tmcG{\tilde{\mathcal{G}}}
\newcommand \tmcH{\tilde{\mathcal{H}}}
\newcommand \tmcI{\tilde{\mathcal{I}}}
\newcommand \tmcJ{\tilde{\mathcal{J}}}
\newcommand \tmcK{\tilde{\mathcal{K}}}
\newcommand \tmcL{\tilde{\mathcal{L}}}
\newcommand \tmcM{\tilde{\mathcal{M}}}
\newcommand \tmcN{\tilde{\mathcal{N}}}
\newcommand \tmcO{\tilde{\mathcal{O}}}
\newcommand \tmcP{\tilde{\mathcal{P}}}
\newcommand \tmcQ{\tilde{\mathcal{Q}}}
\newcommand \tmcR{\tilde{\mathcal{R}}}
\newcommand \tmcS{\tilde{\mathcal{S}}}
\newcommand \tmcT{\tilde{\mathcal{T}}}
\newcommand \tmcU{\tilde{\mathcal{U}}}
\newcommand \tmcV{\tilde{\mathcal{V}}}
\newcommand \tmcW{\tilde{\mathcal{W}}}
\newcommand \tmcX{\tilde{\mathcal{X}}}
\newcommand \tmcY{\tilde{\mathcal{Y}}}
\newcommand \tmcZ{\tilde{\mathcal{Z}}}


%%%% TILDE-BOLD
\newcommand \tba{\tilde{\mathbf{a}}}
\newcommand \tbb{\tilde{\mathbf{b}}}
\newcommand \tbc{\tilde{\mathbf{c}}}
\newcommand \tbd{\tilde{\mathbf{d}}}
\newcommand \tbe{\tilde{\mathbf{e}}}
\newcommand \tbf{\tilde{\mathbf{f}}}
\newcommand \tbh{\tilde{\mathbf{h}}}
\newcommand \tbi{\tilde{\mathbf{i}}}
\newcommand \tbj{\tilde{\mathbf{j}}}
\newcommand \tbk{\tilde{\mathbf{k}}}
\newcommand \tbell{\tilde{\mathbf{\ell}}}
\newcommand \tbm{\tilde{\mathbf{m}}}
\newcommand \tbn{\tilde{\mathbf{n}}}
\newcommand \tbo{\tilde{\mathbf{o}}}
\newcommand \tbp{\tilde{\mathbf{p}}}
\newcommand \tbq{\tilde{\mathbf{q}}}
\newcommand \tbr{\tilde{\mathbf{r}}}
\newcommand \tbs{\tilde{\mathbf{s}}}
\newcommand \tbt{\tilde{\mathbf{t}}}
\newcommand \tbu{\tilde{\mathbf{u}}}
\newcommand \tbv{\tilde{\mathbf{v}}}
\newcommand \tbw{\tilde{\mathbf{w}}}
\newcommand \tbx{\tilde{\mathbf{x}}}
\newcommand \tby{\tilde{\mathbf{y}}}
\newcommand \tbz{\tilde{\mathbf{z}}}
\newcommand \tbA{\tilde{\mathbf{A}}}
\newcommand \tbB{\tilde{\mathbf{B}}}
\newcommand \tbC{\tilde{\mathbf{C}}}
\newcommand \tbD{\tilde{\mathbf{D}}}
\newcommand \tbE{\tilde{\mathbf{E}}}
\newcommand \tbF{\tilde{\mathbf{F}}}
\newcommand \tbG{\tilde{\mathbf{G}}}
\newcommand \tbH{\tilde{\mathbf{H}}}
\newcommand \tbI{\tilde{\mathbf{I}}}
\newcommand \tbJ{\tilde{\mathbf{J}}}
\newcommand \tbK{\tilde{\mathbf{K}}}
\newcommand \tbL{\tilde{\mathbf{L}}}
\newcommand \tbM{\tilde{\mathbf{M}}}
\newcommand \tbN{\tilde{\mathbf{N}}}
\newcommand \tbO{\tilde{\mathbf{O}}}
\newcommand \tbP{\tilde{\mathbf{P}}}
\newcommand \tbQ{\tilde{\mathbf{Q}}}
\newcommand \tbR{\tilde{\mathbf{R}}}
\newcommand \tbS{\tilde{\mathbf{S}}}
\newcommand \tbT{\tilde{\mathbf{T}}}
\newcommand \tbU{\tilde{\mathbf{U}}}
\newcommand \tbV{\tilde{\mathbf{V}}}
\newcommand \tbW{\tilde{\mathbf{W}}}
\newcommand \tbX{\tilde{\mathbf{X}}}
\newcommand \tbY{\tilde{\mathbf{Y}}}
\newcommand \tbZ{\tilde{\mathbf{Z}}}
\newcommand \tbalpha{\tilde{\boldsymbol{\alpha}}}
\newcommand \tbbeta{\tilde{\boldsymbol{\beta}}}
\newcommand \tbgamma{\tilde{\boldsymbol{\gamma}}}
\newcommand \tbdelta{\tilde{\boldsymbol{\delta}}}
\newcommand \tbepsilon{\tilde{\boldsymbol{\epsilon}}}
\newcommand \tbzeta{\tilde{\boldsymbol{\zeta}}}
\newcommand \tbeta{\tilde{\boldsymbol{\eta}}}
\newcommand \tbtheta{\tilde{\boldsymbol{\theta}}}
\newcommand \tbiota{\tilde{\boldsymbol{\iota}}}
\newcommand \tbkappa{\tilde{\boldsymbol{\kappa}}}
\newcommand \tblambda{\tilde{\boldsymbol{\lambda}}}
\newcommand \tbmu{\tilde{\boldsymbol{\mu}}}
\newcommand \tbnu{\tilde{\boldsymbol{\nu}}}
\newcommand \tbxi{\tilde{\boldsymbol{\xi}}}
\newcommand \tbpi{\tilde{\boldsymbol{\pi}}}
\newcommand \tbrho{\tilde{\boldsymbol{\rho}}}
\newcommand \tbsigma{\tilde{\boldsymbol{\sigma}}}
\newcommand \tbtau{\tilde{\boldsymbol{\tau}}}
\newcommand \tbupsilon{\tilde{\boldsymbol{\upsilon}}}
\newcommand \tbphi{\tilde{\boldsymbol{\phi}}}
\newcommand \tbchi{\tilde{\boldsymbol{\chi}}}
\newcommand \tbpsi{\tilde{\boldsymbol{\psi}}}
\newcommand \tbomega{\tilde{\boldsymbol{\omega}}}
\newcommand \tbGamma{\tilde{\mathbf{\Gamma}}}
\newcommand \tbDelta{\tilde{\mathbf{\Delta}}}
\newcommand \tbTheta{\tilde{\mathbf{\Theta}}}
\newcommand \tbLambda{\tilde{\mathbf{\Lambda}}}
\newcommand \tbXi{\tilde{\mathbf{\Xi}}}
\newcommand \tbPi{\tilde{\mathbf{\Pi}}}
\newcommand \tbSigma{\tilde{\mathbf{\Sigma}}}
\newcommand \tbPhi{\tilde{\mathbf{\Phi}}}
\newcommand \tbPsi{\tilde{\mathbf{\Psi}}}
\newcommand \tbOmega{\tilde{\mathbf{\Omega}}}

%%%% CHECK-BOLD
\newcommand \cba{\check{\mathbf{a}}}
\newcommand \cbb{\check{\mathbf{b}}}
\newcommand \cbc{\check{\mathbf{c}}}
\newcommand \cbd{\check{\mathbf{d}}}
\newcommand \cbe{\check{\mathbf{e}}}
\newcommand \cbf{\check{\mathbf{f}}}
\newcommand \cbh{\check{\mathbf{h}}}
\newcommand \cbi{\check{\mathbf{i}}}
\newcommand \cbj{\check{\mathbf{j}}}
\newcommand \cbk{\check{\mathbf{k}}}
\newcommand \cbell{\check{\mathbf{\ell}}}
\newcommand \cbm{\check{\mathbf{m}}}
\newcommand \cbn{\check{\mathbf{n}}}
\newcommand \cbo{\check{\mathbf{o}}}
\newcommand \cbp{\check{\mathbf{p}}}
\newcommand \cbq{\check{\mathbf{q}}}
\newcommand \cbr{\check{\mathbf{r}}}
\newcommand \cbs{\check{\mathbf{s}}}
\newcommand \cbt{\check{\mathbf{t}}}
\newcommand \cbu{\check{\mathbf{u}}}
\newcommand \cbv{\check{\mathbf{v}}}
\newcommand \cbw{\check{\mathbf{w}}}
\newcommand \cbx{\check{\mathbf{x}}}
\newcommand \cby{\check{\mathbf{y}}}
\newcommand \cbz{\check{\mathbf{z}}}
\newcommand \cbA{\check{\mathbf{A}}}
\newcommand \cbB{\check{\mathbf{B}}}
\newcommand \cbC{\check{\mathbf{C}}}
\newcommand \cbD{\check{\mathbf{D}}}
\newcommand \cbE{\check{\mathbf{E}}}
\newcommand \cbF{\check{\mathbf{F}}}
\newcommand \cbG{\check{\mathbf{G}}}
\newcommand \cbH{\check{\mathbf{H}}}
\newcommand \cbI{\check{\mathbf{I}}}
\newcommand \cbK{\check{\mathbf{K}}}
\newcommand \cbL{\check{\mathbf{L}}}
\newcommand \cbM{\check{\mathbf{M}}}
\newcommand \cbN{\check{\mathbf{N}}}
\newcommand \cbO{\check{\mathbf{O}}}
\newcommand \cbP{\check{\mathbf{P}}}
\newcommand \cbQ{\check{\mathbf{Q}}}
\newcommand \cbR{\check{\mathbf{R}}}
\newcommand \cbS{\check{\mathbf{S}}}
\newcommand \cbT{\check{\mathbf{T}}}
\newcommand \cbU{\check{\mathbf{U}}}
\newcommand \cbV{\check{\mathbf{V}}}
\newcommand \cbW{\check{\mathbf{W}}}
\newcommand \cbX{\check{\mathbf{X}}}
\newcommand \cbY{\check{\mathbf{Y}}}
\newcommand \cbZ{\check{\mathbf{Z}}}
\newcommand \cbalpha{\check{\boldsymbol{\alpha}}}
\newcommand \cbbeta{\check{\boldsymbol{\beta}}}
\newcommand \cbgamma{\check{\boldsymbol{\gamma}}}
\newcommand \cbdelta{\check{\boldsymbol{\delta}}}
\newcommand \cbepsilon{\check{\boldsymbol{\epsilon}}}
\newcommand \cbzeta{\check{\boldsymbol{\zeta}}}
\newcommand \cbeta{\check{\boldsymbol{\eta}}}
\newcommand \cbtheta{\check{\boldsymbol{\theta}}}
\newcommand \cbiota{\check{\boldsymbol{\iota}}}
\newcommand \cbkappa{\check{\boldsymbol{\kappa}}}
\newcommand \cblambda{\check{\boldsymbol{\lambda}}}
\newcommand \cbmu{\check{\boldsymbol{\mu}}}
\newcommand \cbnu{\check{\boldsymbol{\nu}}}
\newcommand \cbxi{\check{\boldsymbol{\xi}}}
\newcommand \cbpi{\check{\boldsymbol{\pi}}}
\newcommand \cbrho{\check{\boldsymbol{\rho}}}
\newcommand \cbsigma{\check{\boldsymbol{\sigma}}}
\newcommand \cbtau{\check{\boldsymbol{\tau}}}
\newcommand \cbupsilon{\check{\boldsymbol{\upsilon}}}
\newcommand \cbphi{\check{\boldsymbol{\phi}}}
\newcommand \cbchi{\check{\boldsymbol{\chi}}}
\newcommand \cbpsi{\check{\boldsymbol{\psi}}}
\newcommand \cbomega{\check{\boldsymbol{\omega}}}
\newcommand \cbGamma{\check{\mathbf{\Gamma}}}
\newcommand \cbDelta{\check{\mathbf{\Delta}}}
\newcommand \cbTheta{\check{\mathbf{\Theta}}}
\newcommand \cbLambda{\check{\mathbf{\Lambda}}}
\newcommand \cbXi{\check{\mathbf{\Xi}}}
\newcommand \cbPi{\check{\mathbf{\Pi}}}
\newcommand \cbSigma{\check{\mathbf{\Sigma}}}
\newcommand \cbPhi{\check{\mathbf{\Phi}}}
\newcommand \cbPsi{\check{\mathbf{\Psi}}}
\newcommand \cbOmega{\check{\mathbf{\Omega}}}

%% HAT-BOLD
\newcommand \hba{\hat{\mathbf{a}}}
\newcommand \hbb{\hat{\mathbf{b}}}
\newcommand \hbc{\hat{\mathbf{c}}}
\newcommand \hbd{\hat{\mathbf{d}}}
\newcommand \hbe{\hat{\mathbf{e}}}
\newcommand \hbf{\hat{\mathbf{f}}}
\newcommand \hbh{\hat{\mathbf{h}}}
\newcommand \hbi{\hat{\mathbf{i}}}
\newcommand \hbj{\hat{\mathbf{j}}}
\newcommand \hbk{\hat{\mathbf{k}}}
\newcommand \hbell{\hat{\mathbf{\ell}}}
\newcommand \hbm{\hat{\mathbf{m}}}
\newcommand \hbn{\hat{\mathbf{n}}}
\newcommand \hbo{\hat{\mathbf{o}}}
\newcommand \hbp{\hat{\mathbf{p}}}
\newcommand \hbq{\hat{\mathbf{q}}}
\newcommand \hbr{\hat{\mathbf{r}}}
\newcommand \hbs{\hat{\mathbf{s}}}
\newcommand \hbt{\hat{\mathbf{t}}}
\newcommand \hbu{\hat{\mathbf{u}}}
\newcommand \hbv{\hat{\mathbf{v}}}
\newcommand \hbw{\hat{\mathbf{w}}}
\newcommand \hbx{\hat{\mathbf{x}}}
\newcommand \hby{\hat{\mathbf{y}}}
\newcommand \hbz{\hat{\mathbf{z}}}
\newcommand \hbA{\hat{\mathbf{A}}}
\newcommand \hbB{\hat{\mathbf{B}}}
\newcommand \hbC{\hat{\mathbf{C}}}
\newcommand \hbD{\hat{\mathbf{D}}}
\newcommand \hbE{\hat{\mathbf{E}}}
\newcommand \hbF{\hat{\mathbf{F}}}
\newcommand \hbG{\hat{\mathbf{G}}}
\newcommand \hbH{\hat{\mathbf{H}}}
\newcommand \hbI{\hat{\mathbf{I}}}
\newcommand \hbK{\hat{\mathbf{K}}}
\newcommand \hbL{\hat{\mathbf{L}}}
\newcommand \hbM{\hat{\mathbf{M}}}
\newcommand \hbN{\hat{\mathbf{N}}}
\newcommand \hbO{\hat{\mathbf{O}}}
\newcommand \hbP{\hat{\mathbf{P}}}
\newcommand \hbQ{\hat{\mathbf{Q}}}
\newcommand \hbR{\hat{\mathbf{R}}}
\newcommand \hbS{\hat{\mathbf{S}}}
\newcommand \hbT{\hat{\mathbf{T}}}
\newcommand \hbU{\hat{\mathbf{U}}}
\newcommand \hbV{\hat{\mathbf{V}}}
\newcommand \hbW{\hat{\mathbf{W}}}
\newcommand \hbX{\hat{\mathbf{X}}}
\newcommand \hbY{\hat{\mathbf{Y}}}
\newcommand \hbZ{\hat{\mathbf{Z}}}
\newcommand \hbalpha{\hat{\boldsymbol{\alpha}}}
\newcommand \hbbeta{\hat{\boldsymbol{\beta}}}
\newcommand \hbgamma{\hat{\boldsymbol{\gamma}}}
\newcommand \hbdelta{\hat{\boldsymbol{\delta}}}
\newcommand \hbepsilon{\hat{\boldsymbol{\epsilon}}}
\newcommand \hbzeta{\hat{\boldsymbol{\zeta}}}
\newcommand \hbeta{\hat{\boldsymbol{\eta}}}
\newcommand \hbtheta{\hat{\boldsymbol{\theta}}}
\newcommand \hbiota{\hat{\boldsymbol{\iota}}}
\newcommand \hbkappa{\hat{\boldsymbol{\kappa}}}
\newcommand \hblambda{\hat{\boldsymbol{\lambda}}}
\newcommand \hbmu{\hat{\boldsymbol{\mu}}}
\newcommand \hbnu{\hat{\boldsymbol{\nu}}}
\newcommand \hbxi{\hat{\boldsymbol{\xi}}}
\newcommand \hbpi{\hat{\boldsymbol{\pi}}}
\newcommand \hbrho{\hat{\boldsymbol{\rho}}}
\newcommand \hbsigma{\hat{\boldsymbol{\sigma}}}
\newcommand \hbtau{\hat{\boldsymbol{\tau}}}
\newcommand \hbupsilon{\hat{\boldsymbol{\upsilon}}}
\newcommand \hbphi{\hat{\boldsymbol{\phi}}}
\newcommand \hbchi{\hat{\boldsymbol{\chi}}}
\newcommand \hbpsi{\hat{\boldsymbol{\psi}}}
\newcommand \hbomega{\hat{\boldsymbol{\omega}}}
\newcommand \hbGamma{\hat{\mathbf{\Gamma}}}
\newcommand \hbDelta{\hat{\mathbf{\Delta}}}
\newcommand \hbTheta{\hat{\mathbf{\Theta}}}
\newcommand \hbLambda{\hat{\mathbf{\Lambda}}}
\newcommand \hbXi{\hat{\mathbf{\Xi}}}
\newcommand \hbPi{\hat{\mathbf{\Pi}}}
\newcommand \hbSigma{\hat{\mathbf{\Sigma}}}
\newcommand \hbPhi{\hat{\mathbf{\Phi}}}
\newcommand \hbPsi{\hat{\mathbf{\Psi}}}
\newcommand \hbOmega{\hat{\mathbf{\Omega}}}

%% BAR-BOLD
\newcommand \bba{\bar{\mathbf{a}}}
\newcommand \bbb{\bar{\mathbf{b}}}
\newcommand \bbc{\bar{\mathbf{c}}}
\newcommand \bbd{\bar{\mathbf{d}}}
\newcommand \bbe{\bar{\mathbf{e}}}
\newcommand \bbf{\bar{\mathbf{f}}}
\newcommand \bbh{\bar{\mathbf{h}}}
\newcommand \bbi{\bar{\mathbf{i}}}
\newcommand \bbj{\bar{\mathbf{j}}}
\newcommand \bbk{\bar{\mathbf{k}}}
\newcommand \bbell{\bar{\mathbf{\ell}}}
\newcommand \bbm{\bar{\mathbf{m}}}
\newcommand \bbn{\bar{\mathbf{n}}}
\newcommand \bbo{\bar{\mathbf{o}}}
\newcommand \bbp{\bar{\mathbf{p}}}
\newcommand \bbq{\bar{\mathbf{q}}}
\newcommand \bbr{\bar{\mathbf{r}}}
\newcommand \bbs{\bar{\mathbf{s}}}
\newcommand \bbt{\bar{\mathbf{t}}}
\newcommand \bbu{\bar{\mathbf{u}}}
\newcommand \bbv{\bar{\mathbf{v}}}
\newcommand \bbw{\bar{\mathbf{w}}}
\newcommand \bbx{\bar{\mathbf{x}}}
\newcommand \bby{\bar{\mathbf{y}}}
\newcommand \bbz{\bar{\mathbf{z}}}
\newcommand \bbA{\bar{\mathbf{A}}}
\newcommand \bbB{\bar{\mathbf{B}}}
\newcommand \bbC{\bar{\mathbf{C}}}
\newcommand \bbD{\bar{\mathbf{D}}}
\newcommand \bbE{\bar{\mathbf{E}}}
\newcommand \bbF{\bar{\mathbf{F}}}
\newcommand \bbG{\bar{\mathbf{G}}}
\newcommand \bbH{\bar{\mathbf{H}}}
\newcommand \bbI{\bar{\mathbf{I}}}
\newcommand \bbJ{\bar{\mathbf{J}}}
\newcommand \bbK{\bar{\mathbf{K}}}
\newcommand \bbL{\bar{\mathbf{L}}}
\newcommand \bbM{\bar{\mathbf{M}}}
\newcommand \bbN{\bar{\mathbf{N}}}
\newcommand \bbO{\bar{\mathbf{O}}}
\newcommand \bbP{\bar{\mathbf{P}}}
\newcommand \bbQ{\bar{\mathbf{Q}}}
\newcommand \bbR{\bar{\mathbf{R}}}
\newcommand \bbS{\bar{\mathbf{S}}}
\newcommand \bbT{\bar{\mathbf{T}}}
\newcommand \bbU{\bar{\mathbf{U}}}
\newcommand \bbV{\bar{\mathbf{V}}}
\newcommand \bbW{\bar{\mathbf{W}}}
\newcommand \bbX{\bar{\mathbf{X}}}
\newcommand \bbY{\bar{\mathbf{Y}}}
\newcommand \bbZ{\bar{\mathbf{Z}}}
\newcommand \bbalpha{\bar{\boldsymbol{\alpha}}}
\newcommand \bbbeta{\bar{\boldsymbol{\beta}}}
\newcommand \bbgamma{\bar{\boldsymbol{\gamma}}}
\newcommand \bbdelta{\bar{\boldsymbol{\delta}}}
\newcommand \bbepsilon{\bar{\boldsymbol{\epsilon}}}
\newcommand \bbzeta{\bar{\boldsymbol{\zeta}}}
\newcommand \bbtheta{\bar{\boldsymbol{\theta}}}
\newcommand \bbiota{\bar{\boldsymbol{\iota}}}
\newcommand \bbkappa{\bar{\boldsymbol{\kappa}}}
\newcommand \bblambda{\bar{\boldsymbol{\lambda}}}
\newcommand \bbmu{\bar{\boldsymbol{\mu}}}
\newcommand \bbnu{\bar{\boldsymbol{\nu}}}
\newcommand \bbxi{\bar{\boldsymbol{\xi}}}
\newcommand \bbpi{\bar{\boldsymbol{\pi}}}
\newcommand \bbrho{\bar{\boldsymbol{\rho}}}
\newcommand \bbsigma{\bar{\boldsymbol{\sigma}}}
\newcommand \bbtau{\bar{\boldsymbol{\tau}}}
\newcommand \bbupsilon{\bar{\boldsymbol{\upsilon}}}
\newcommand \bbphi{\bar{\boldsymbol{\phi}}}
\newcommand \bbchi{\bar{\boldsymbol{\chi}}}
\newcommand \bbpsi{\bar{\boldsymbol{\psi}}}
\newcommand \bbomega{\bar{\boldsymbol{\omega}}}
\newcommand \bbGamma{\bar{\mathbf{\Gamma}}}
\newcommand \bbDelta{\bar{\mathbf{\Delta}}}
\newcommand \bbTheta{\bar{\mathbf{\Theta}}}
\newcommand \bbLambda{\bar{\mathbf{\Lambda}}}
\newcommand \bbXi{\bar{\mathbf{\Xi}}}
\newcommand \bbPi{\bar{\mathbf{\Pi}}}
\newcommand \bbSigma{\bar{\mathbf{\Sigma}}}
\newcommand \bbPhi{\bar{\mathbf{\Phi}}}
\newcommand \bbPsi{\bar{\mathbf{\Psi}}}
\newcommand \bbOmega{\bar{\mathbf{\Omega}}}

%%%%%%%%%%%%%%%%DOT_BOLD
\newcommand \bdk{\dot{\mathbf{k}}}
\newcommand \bdK{\dot{\mathbf{K}}}

\newcommand \bdy{\dot{\mathbf{y}}}
\newcommand \bdY{\dot{\mathbf{Y}}}


%%%%%%%%%%%%%%%% HAT_DOT_BOLD
\newcommand \hbdy{\hat{\dot{\mathbf{y}}}}
\newcommand \hbdY{\hat{\dot{\mathbf{Y}}}}

==> myabrv.tex <==
%%
%% IEEEabrv.bib
%% 
%% BibTeX bibliography string definitions of the ABBREVIATED titles of
%% IEEE journals and magazines
%% 
%% NOTE: This text file uses UNIX line feed conventions. When (human)
%% reading this file on other platforms, you may have to use a text
%% editor that can handle lines terminated by the UNIX line feed
%% character (0x0A).
%% 
%% This file is designed for bibliography styles that require TSP
%% abbreviated titles and is not for use in bibliographies that
%% require full-length titles.
%% 
%% Version 1.10 (2003/04/02power
)
%% 
%% Composed by Michael Shell
%% 
%% See:
%% http://www.ctan.org/tex-archive/macros/latex/contrib/supported/IEEEtran/
%% for latest version and current contact information.
%%
%% Special thanks to Laura Hyslop of IEEE for her help in obtaining the
%% information needed to compile this file. Also, Volker Kuhlmann kindly
%% provided some corrections and additions.
%%
%%**********************************************************************
%% Legal Notice:
%% This code is offered as-is without any warranty either expressed or
%% implied; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE!
%% User assumes all risk.
%% In no event shall IEEE or any contributor to this code be liable for
%% any damages or losses, including, but not limited to, incidental,
%% consequential, or any other damages, resulting from the use or misuse
%% of any information contained here.
%%
%% This code is distributed under the Perl Artistic License 
%% ( http://language.perl.com/misc/Artistic.html ) 
%% and may be freely used, distributed and modified - subject to the
%% constraints therein.
%% Retain all contribution notices, credits and disclaimers.
%% 
%% All comments are the opinions of their respective authors and are not
%% necessarily endorsed by the IEEE.
%%**********************************************************************
%
%
% USAGE:
% 
% \bibliographystyle{mybstfile} 
% \bibliography{IEEEabrv,mybibfile}
%
% where the IEEE titles in the .bib database entries use the strings
% defined here. e.g.,
%
%
%    journal = IEEE_J_AC,
%
%
% to yield "{IEEE} Trans. Automat. Contr."
%
%
% IEEE uses abbreviated journal titles in their bibliographies -
% this file is suitable for work that is to be submitted to the IEEE.
%
%
% For work that requires full-length titles, you should use the full
% titles provided in the companion file, IEEEfull.bib.
%
%
% ** NOTES **
%
% 1. Journals have been grouped according to subject in order to make it
%    easier to locate and extract the definitions for related journals - 
%    as most works use references that are confined to a single topic.
%    Magazines are listed in straight alphabetical order.
%
% 2. String names are closely based on IEEE's own internal acronyms.
% 
% 3. Abbreviations follow IEEE's style.
%
% 4. Older, out-of-print IEEE titles are included (but not including titles
%    dating prior to IEEE's formation from the IRE and AIEE in 1963).
%
% 5. The following NEW/current journal definitions have been disabled because
%    their abbreviations have not yet been finalized/verified:
%    
%    STRING{IEEE_J_MC         = "{IEEE} Trans. Mobile Comput."}
%    STRING{IEEE_J_JEM        = "{IEEE/TMS} J. Electron. Mater."}
%    STRING{IEEE_J_MCTE       = "{IEEE} Trans. Molecular Cellular Tissue Eng."}
%    STRING{IEEE_J_ESSL       = "{IEEE/ECS} Electrochemical Solid-State Lett."}
%    STRING{IEEE_J_CJECE      = "Canadian J. Elect. Comput. Eng."}
%    
% 6. The following OLD journal definitions have been disabled because
%    their abbreviations have not yet been found/verified:
%
%    STRING{IEEE_J_EWS        = "{IEEE} Trans. Eng. Writing Speech"}
%    STRING{IEEE_J_BCTV       = "{IEEE} Trans. Broadcast Television Receivers"}
%
% If you know what the proper abbreviation is for a string in #5 or #6 above,
% email me and I will correct them in the next release.

%%%%%%%%%%%%%%%%%%%%%%
%% IEEE Conferences %%
%%%%%%%%%%%%%%%%%%%%%%

% power
@STRING{IEEE_C_NAPS   	= "Proc. North American Power Symposium"}
@STRING{IEEE_C_ISGT    	= "Proc. {IEEE} Conf. on Innovative Smart Grid Technologies"}
@STRING{IEEE_C_GM      	= "Proc. {IEEE} Power \& Energy Society General Meeting"}
@STRING{IEEE_C_SGC    	= "Proc. {IEEE} Intl. Conf. on Smart Grid Commun."}
@STRING{PSCC     		= "Proc. Power Syst. Comput. Conf."}
@STRING{C_ALLERTON     = "Proc. Allerton Conf. on Comm., Control, and Computing"}


% signal processing
@STRING{IEEE_C_ICASSP    = "Proc. {IEEE} Intl. Conf. on Acoustics, Speech, and Signal Process."}
@STRING{C_Asilomar    = "Proc. {Asilomar} Conf. on Signals, Syst. and Comput."}
@STRING{IEEE_C_GLOBALSIP    = "Proc. {IEEE} Global Conf. on Signal and Inf. Process."}
@STRING{IEEE_C_CAMSAP    = "Proc. {IEEE} Wkshp. on Comp. Adv. in Multi-Sensor Adaptive Proc."}

% communications

% control
@STRING{IEEE_C_CDC    	= "Proc. {IEEE} Conf. on Decision and Control"}
@STRING{C_ACC			= "Proc. American Control Conf."}

@STRING{JMLR			= "{J. of Machine Learning Research}"}

%%%%%%%%%%%%%%%%%%%
%% IEEE Journals %%
%%%%%%%%%%%%%%%%%%%

% aerospace and military
@STRING{IEEE_J_AES        = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE        = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_ANNE       = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AS         = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE       = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL        = "{IEEE} Trans. Mil. Electron."}



% autos, transportation and vehicles (non-aerospace)
@STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transport. Syst."}
@STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}



% circuits, signals, systems, audio and controls
@STRING{IEEE_J_SPL        = "{IEEE} Signal Process. Lett."}
@STRING{IEEE_J_ASSP       = "{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_AC         = "{IEEE} Trans. Autom. Contr."}
@STRING{IEEE_J_CNS         = "{IEEE} Trans. Control Netw. Syst."}
@STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT         = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST        = "{IEEE} Trans. Contr. Syst. Technol."}
@STRING{IEEE_J_SP         = "{IEEE} Trans. Signal Process."}
@STRING{IEEE_J_STSP       = "{IEEE} J. Sel. Topics Signal Process."}
@STRING{IEEE_J_SU         = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP        = "{IEEE} Trans. Speech Audio Process."}
@STRING{IEEE_J_UE         = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC       = "{IEEE} Trans. Ultrason., Ferroelect., Freq. Contr."}



% communications
@STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC       = "{IEEE} J. Select. Areas Commun."}
@STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}



% components, packaging and manufacturing
@STRING{IEEE_J_ADVP       = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT       = "{IEEE} Trans. Comp., Hybrids, Manufact. Technol."}
@STRING{IEEE_J_CPMTA      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {A}"}
@STRING{IEEE_J_CPMTB      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {B}"}
@STRING{IEEE_J_CPMTC      = "{IEEE} Trans. Comp., Packag., Manufact. Technol. {C}"}
@STRING{IEEE_J_CAPT       = "{IEEE} Trans. Comp. Packag. Technol."}
@STRING{IEEE_J_CAPTS      = "{IEEE} Trans. Comp. Packag. Technol."}
@STRING{IEEE_J_CPART      = "{IEEE} Trans. Comp. Parts"}
@STRING{IEEE_J_EPM        = "{IEEE} Trans. Electron. Packag. Manufact."}
@STRING{IEEE_J_MFT        = "{IEEE} Trans. Manufact. Technol."}
@STRING{IEEE_J_PHP        = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP        = "{IEEE} Trans. Parts, Mater., Packag."}



% CAD
@STRING{IEEE_J_TCAD       = "{IEEE} J. Technol. Computer Aided Design"}
@STRING{IEEE_J_CAD        = "{IEEE} Trans. Computer-Aided Design"}



% coding, data, information, knowledge
@STRING{IEEE_J_IT         = "{IEEE} Trans. Inf. Theory"}
@STRING{IEEE_J_KDE        = "{IEEE} Trans. Knowl. Data Eng."}



% computers, computation, networking and software
@STRING{IEEE_J_C          = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_ECOMP      = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_EVC        = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ       = "{IEEE} Trans. Fuzzy Syst."}
% disabled till definition finalized
STRING{IEEE_J_MC          = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_NET        = "{IEEE/ACM} Trans. Netw."}
@STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Netw."}
@STRING{IEEE_J_PDS        = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SE         = "{IEEE} Trans. Softw. Eng."}



% computer graphics, imaging, and multimedia
@STRING{IEEE_J_IP         = "{IEEE} Trans. Image Process."}
@STRING{IEEE_J_MM         = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG        = "{IEEE} Trans. Vis. Comput. Graphics"}



% cybernetics, ergonomics, robots, man-machine, and automation
@STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
@STRING{IEEE_J_RA         = "{IEEE} Trans. Robot. Autom."}
@STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SSC        = "{IEEE} Trans. Syst. Sci. Cybern."}



% earth, wind, fire and water
@STRING{IEEE_J_GE         = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS        = "{IEEE} Trans. Geosci. Remote Sens."}
@STRING{IEEE_J_OE         = "{IEEE} J. Ocean. Eng."}



% education, engineering, history, IEEE, professional
% disabled till definition is verified
STRING{IEEE_J_CJECE       = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC       = "Proc. {IEEE}"}  %%% Proceedings of the IEEE 
@STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM         = "{IEEE} Trans. Eng. Manage."}
% disabled till definition is verified
STRING{IEEE_J_EWS         = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}



% electromagnetics, antennas, EMI, magnetics and microwave
@STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propagat. Lett."}
@STRING{IEEE_J_MGWL       = "{IEEE} Microwave Guided Wave Lett."}
% IEEE seems to want "Compon." here, not "Comp."
@STRING{IEEE_J_MWCL       = "{IEEE} Microwave Wireless Compon. Lett."}
@STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas Propagat."}
@STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT        = "{IEEE} Trans. Microwave Theory Tech."}
@STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J. Magn. Jpn."}



% energy and power
@STRING{IEEE_J_EC         = "{IEEE} Trans. Energy Convers."}	% 2.43
@STRING{IEEE_J_PWRAS      = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD       = "{IEEE} Trans. Power Del."}	% 1.52 	
@STRING{IEEE_J_PWRE       = "{IEEE} Trans. Power Electron."}	% 4.08
@STRING{IEEE_J_PWRS       = "{IEEE} Trans. Power Syst."}		% 2.92
@STRING{IEEE_J_SG 	      = "{IEEE} Trans. Smart Grid"}
@STRING{IEEE_J_STE 	      = "{IEEE} Trans. Sustain. Energy"}


% industrial, commercial and consumer
@STRING{IEEE_J_APPIND     = "{IEEE} Trans. Applicat. Ind."}
@STRING{IEEE_J_BC         = "{IEEE} Trans. Broadcast."}
% disabled till definition is verified
STRING{IEEE_J_BCTV        = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE         = "{IEEE} Trans. Consumer Electron."}
@STRING{IEEE_J_IE         = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI       = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Applicat."}
@STRING{IEEE_J_IGA        = "{IEEE} Trans. Ind. Gen. Applicat."}



% instrumentation and measurement
@STRING{IEEE_J_IM         = "{IEEE} Trans. Instrum. Meas."}



% insulation and materials
% disabled till definition finalized
STRING{IEEE_J_JEM         = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI        = "{IEEE} Trans. Dielect. Elect. Insulation"}
@STRING{IEEE_J_EI         = "{IEEE} Trans. Elect. Insulation"}



% mechanical
@STRING{IEEE_J_MECH       = "{IEEE/ASME} Trans. Mechatron."}
@STRING{IEEE_J_MEMS       = "J. Microelectromech. Syst."}



% medical and biological
@STRING{IEEE_J_BME        = "{IEEE} Trans. Biomed. Eng."}
% Note: The B-ME journal later dropped the hyphen and became the BME.
@STRING{IEEE_J_B-ME       = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_BMELC      = "{IEEE} Trans. Bio-Med. Electron."}
@STRING{IEEE_J_ITBM       = "{IEEE} Trans. Inf. Technol. Biomed."}
@STRING{IEEE_J_ME         = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI         = "{IEEE} Trans. Med. Imag."}
% disabled till definition finalized
STRING{IEEE_J_MCTE        = "{IEEE} Trans. Molecular Cellular Tissue Eng."}
@STRING{IEEE_J_NB         = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE       = "{IEEE} Trans. Neural Syst. Rehab. Eng."}
@STRING{IEEE_J_RE         = "{IEEE} Trans. Rehab. Eng."}



% optics, lightwave and photonics
@STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_JLT        = "J. Lightwave Technol."}



% physics, electrons, nanotechnology, nuclear and quantum electronics
@STRING{IEEE_J_EDL        = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_JQE        = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE      = "{IEEE} J. Select. Topics Quantum Electron."}
@STRING{IEEE_J_ED         = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO       = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS         = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS         = "{IEEE} Trans. Plasma Sci."}



% reliability
% IEEE seems to want "Mat." here, not "Mater."
@STRING{IEEE_J_DMR        = "{IEEE} Trans. Device Mat. Rel."}
@STRING{IEEE_J_R          = "{IEEE} Trans. Rel."}



% semiconductors, superconductors, electrochemical and solid state
% disabled till definition finalized
STRING{IEEE_J_ESSL        = "{IEEE/ECS} Electrochemical Solid-State Lett."}
@STRING{IEEE_J_JSSC       = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC        = "{IEEE} Trans. Appl. Superconduct."}
@STRING{IEEE_J_SM         = "{IEEE} Trans. Semiconduct. Manufact."}



% sensors
@STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}



% VLSI
@STRING{IEEE_J_VLSI       = "{IEEE} Trans. {VLSI} Syst."}





%%%%%%%%%%%%%%%%%%%%
%% IEEE Magazines %%
%%%%%%%%%%%%%%%%%%%%


@STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag"}
@STRING{IEEE_M_HIST       = "{IEEE} Annals Hist. Comput."}
@STRING{IEEE_M_AP         = "{IEEE} Antennas Propagat. Mag."}
@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}
% CSEM changed to CSE in 1999
@STRING{IEEE_M_CSE        = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C          = "{IEEE} Computer"}
@STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EXP        = "{IEEE} Expert"}
@STRING{IEEE_M_IA         = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IM         = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
@STRING{IEEE_M_MW         = "{IEEE} Microwave"}
@STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
@STRING{IEEE_M_NET        = "{IEEE} Network"}
% IEEE's editorial manual lists "Pers. Commun.", 
% but "Personal Commun. Mag." seems to be what is used in the journals
@STRING{IEEE_M_PCOM       = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_POT        = "{IEEE} Potentials"}
% CAP and PER merged to form PE in 2003
@STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_RA         = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SP         = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S          = "{IEEE} Softw."}
@STRING{IEEE_M_SPECT      = "{IEEE} Spectr."}
@STRING{IEEE_M_TS         = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_WC         = "{IEEE} Wireless Commun. Mag."}
@STRING{IEEE_M_TODAY      = "Today's Eng."}




%--
%EOF

